A Comprehensive Evaluation of Android ICC Resolution Techniques

Inter-component communication (ICC) is a widely used mechanism in mobile apps, which enables message-based control flow transferring and data passing between Android components. Effective ICC resolution requires precisely identifying entry points, analyzing data values of ICC fields, modeling related framework APIs, etc. Due to various control-flow- and data-flow-related characteristics involved and the lack of oracles for real-world apps, the comprehensive evaluation of ICC resolution techniques is challenging. To fill this gap, we collect multiple-type benchmark suites with 4,104 apps, covering hand-made apps, open-source, and commercial ones. Considering their differences, various evaluation metrics, e.g., number count, graph structure, and reliable oracle based metrics, are adopted on-demand. As the oracle for real-world apps is unavailable, we design a dynamic analysis approach to extract the real ICC links triggered during GUI exploration. By auditing the code implementations, we carefully check the extracted ICCs and confirm 1,680 ones to form a reliable oracle set, in which each ICC is labeled with 25 code characteristic tags. The evaluation performed on six state-of-the-art ICC resolution tools shows that 1) the completeness of static ICC resolution results on real-world apps is not satisfactory, as up to 38%-85% ICCs are missed by tools; 2) many wrongly reported ICCs are sent from or received by only a few components and the graph structure information can help the identification; 3) the efficiency of fundamental tools, like ICC resolution ones, should be optimized in both engineering and research aspects. By investigating both the missed and wrongly reported ICCs, we discuss the strengths of different tools for users and summarize eight common FN/FP patterns in ICC resolution for tool developers.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> content/implementation.tex <==

\section{Enhancing ICC Resolution Ability}
According to our investigation, with various ICC resolution tools available, more than half of the ICCs are missed.
If the apps which failed the analysis are taken into consideration, the FN rate become much higher. 
By the root cause analysis, we noticed that \textbf{the implicit control flow, specific modeling of Android components and ICC behavior, as well as the context-sensitive data-flow analysis} are the key factors that influence the resolution results.
In addition, the tool should concern the usability and the reliability on complex real-world apps.
Thus, we aim to design a characteristic-directed ICC resolution tool with extra attention to its efficiency.

% In this section, we propose an ICC resolution tool, \textit{ICCBot}, whose design is based on the key characteristics discussed above.

\subsection{Characteristic-Directed ICC Resolution}
%  \textcolor{blue}{and carrying a set of configurable switches for characteristic selection}.

\begin{figure}[!tb]
	\setlength{\abovecaptionskip}{5pt}
	\setlength{\belowcaptionskip}{-20pt}
	\centering
	\includegraphics[width=0.47\textwidth]{fig/implement.pdf}
	\caption{Framework of ICCBot}
	\label{fig:Implementation}
\end{figure}

Fig.~\ref{fig:Implementation} presents the overview of our ICC resolution approach, which contains three main modules: 1) control-flow, 2) data-flow, and 3) object model analysis.
For control-flow analysis, dummy main and callback analysis modules provided by FlowDroid~\cite{Arzt14PLDI} are adopted to construct the initial set of CG edges and callback entries.
Based on it, the asynchronous and polymorphic related call edges and the user-customized callback listeners are recognized to enhance them. 
For data-flow analysis, we adopt the intra-procedural reaching definition analysis~\cite{PPA} to get the target object related \textit{du-chains} in each method and perform an inter-procedural context-sensitive analysis to track the data values transferred among methods.
For the object model module, we mainly focus on modeling two types of objects: 1) \texttt{Fragment} modeling is essential to control-flow enhancing, and 2) \texttt{Intent} modeling is essential to ICC message analysis.
We model the behaviors of the related APIs according to their semantics and identify the objects whose behavior successfully triggers \texttt{Fragment} loading and \texttt{Intent} sending. 

% \vspace{-0.3cm}

\subsection{Summary-Based Analysis}
An observation from literature~\cite{DBLP:conf/ccs/BosuLYW17} is that the reliability and the usability of tools when they analyze complex apps are important concerns.
To improve analysis efficiency, we consider building lightweight summaries for each method, object, 
and component to achieve ICC resolution while reducing unnecessary computation.

\textbf{Method Summary.} 
The summary of a method can be formally defined as a triple $\mathcal{MS}=\langle mtd, S_{os}, S_{ms} \rangle$, where
\begin{itemize}[leftmargin=10pt]
	\item $mtd$ is the unique signature of current method.
	\item $S_{os}$ is a set of object summaries. Each $os \in S_{os}$ is an object summary whose intent or fragment object is operated in $mtd$.
	\item $S_{ms}$ is a set of method summaries. Each $ms \in S_{ms}$ denotes a callee method who does not carry objects that relevant with~$mtd$. 
\end{itemize}
Each method summary contains a set of object summaries and a set of callee method summaries. The analysis is in a bottom-up order according to an acyclic CG, in which the cycles are removed by a pre-processing.
The object summary set $S_{os}$ includes the newly created \texttt{Intent/Fragment} objects in the current method.
For the callees that passing out or returning a concerned object or its filed value, we make inter-procedure and context-sensitive analysis to get the corresponding object summary.
And for other callees whose object usage is irrelevant with method $mtd$, their method summaries are directly added into the set $S_{ms}$, which avoids re-analysis.
For each method, the summaries are built path-sensitively and the max number of paths under analysis can be limited with a threshold to avoid the path exploration problem.


\textbf{Object Summary.} The object summary achieves the behavior modeling of \texttt{Intent} or \texttt{Fragment} objects, which contains the object operating statements in a path. We group the statements into three categories and manipulate the object instance according to the operation and data of each statement.
For example, the statement \texttt{i = new Intent()} create Intent object \texttt{i} and 
the statement \texttt{i.addAction(s)} updates the field value of \texttt{i}.
The summary of an \texttt{Intent} or \texttt{Fragment} object can be formally defined as a 6-tuple $\mathcal{OS} = \langle obj, mtd, L_{smt}, L_{create}, M_{update}, L_{send} \rangle$, where

\begin{itemize}[leftmargin=10pt]
	\item $obj$ is an object instance to be modeled.
	\item $mtd$ is the signature of method that object $obj$ belongs to.
	\item $L_{smt}$ is a list of statements that related to the usage of $obj$, which is path sensitively generated.
	\item $L_{create} \subset L_{smt}$ is a list of object creating or receiving related statements that creates object $obj$, $|L_{create}| = 1$.
	\item $L_{update} \subset L_{smt}$ is a list of object updating related statements, each statement is used to update the field of object $obj$.
	\item $L_{send} \subset L_{smt}$ is a list of object sending related statements, which delivers object $obj$ to Android framework, $|L_{send}| = 1$.
\end{itemize}

\textbf{Component Summary.} Based on the object summaries, we can obtain the fragment loading relationship to enhance CG, and extract the source or destination information to resolve ICC links.
The summary of a component can be formally defined as a triple $\mathcal{CS}=\langle source, S_{destination}, S_{obj} \rangle$, where

\begin{itemize}[leftmargin=10pt]
	\item $source$ is the component that sending out the target object.
	\item $S_{destination}$ is a set of components to be launched.
	\item $S_{obj}$ is a set of object summaries, each of which describes the behavior of an object.
\end{itemize}

A set of ICCs could be collected based on these summaries. For implicit Intents, the Intent fields are matched with the declared intent-filters to get target addresses.
Besides, values of the destination irrelevant fields are also extracted to describe an ICC.

\subsection{Evaluation on the Three Benchmarks}
We then evaluate \textit{ICCBot} on the three benchmarks provided previously.
On benchmark I, \textit{ICCBot} outperforms others with a 98\% resolution precision in total, in which the two FNs are caused by unmodeled library APIs.
On benchmark II, \textit{ICCBot} can successfully analyze all the apps and it recognizes 20,942 and 74,888 ICCs on the F-droid and the Google Play datasets, respectively.
Besides, it achieves the highest completeness value 0.77 while the value of connectivity$_{cpt}$ is less than three, which may benefit from the multiple characteristics-directed analysis.
For the evaluation with the 31 apps, ICCBot successfully resolves 2,603 ICC for all these apps, and the analyzing time is 230s on average.
Its constructed CTG has a completeness 0.66, connectivity 4.62, and connectivity$_{cpt}$ 7.02.
Compared with the PRR oracle, it misses 574 ICCs and the average FN rate for all apps is 26.4\%.  
Most of the FNs are related to the unmodeled Atypical ICC, library and complex call context.
Overall, the characteristic-directed tool design and the summary-based program analysis helps to improve the ICC resolution ability significantly.
More evaluation details are available at~\cite{ICC-Resolution-Evaluation}.

% And for tool \textit{ICCBot}, the top apps are \textit{SuntimesWidget} (17.2) and \textit{Osmand} (16.3),
% in which \textit{SuntimesWidget} is an app with multiple widgets and there are massive broadcast messages among them. And \textit{Osmand} is full of fragment transitions, so that the FPs are related to the path feasibility, which is unmodeled in all the approaches.

==> content/related.tex <==
\section{Related Work}
% To the best of our knowledge, we have presented the first oracle construction approach for the ICC message resolution circumstance, 
% which provides a more practical ICC resolution evaluation and feedback on the hand-made benchmark construction.
% The motivation of our approach is that the existing research literature has proposed a large body of works focusing on applying Android ICC,
% whose effectiveness is limited by the precision of ICC resolution tools.
% However, the weakness of state-of-the-art tools on real-world apps is unclear up to now.

\textbf{ICC Resolution Application Scenarios.}
Existing researchers have proposed many works that apply the Android ICC resolution results.
One of the most popular application scenarios is security property checking, especially privacy leak detection.
In the beginning, the intra-component leak detection is concerned by teams like \textit{FlowDroid}~\cite{Arzt14PLDI}, \textit{LeakMiner}~\cite{Leakminer} and \textit{Scandal}~\cite{SCANDAL}.
Considering that sensitive data can be passed by ICC links, several researchers extend the approaches to support inter-component leak detection, including \textit{IccTA}~\cite{Li15ICSE},
\textit{Amandroid}~\cite{DBLP:conf/ccs/WeiROR14} and \textit{DroidSafe}~\cite{DBLP:conf/ndss/GordonKPGNR15}.
Among these tools, the ICC resolution ability of \textit{IccTA} depends on the state-of-the-art tool \textit{IC3}, while \textit{Amandroid}~\cite{DBLP:conf/ccs/WeiROR14} and \textit{DroidSafe}~\cite{DBLP:conf/ndss/GordonKPGNR15} manually built a precise model for intent manipulation APIs.
Besides privacy leak, ICC resolution also relates to malware detection~\cite{DBLP:journals/tifs/XuLD16}, inter-app threat analysis~\cite{DBLP:conf/ccs/BosuLYW17, DBLP:journals/tmc/ElishCBYR20,DBLP:journals/fgcs/BhandariHLZGR20}, etc.
Another typical scenario is GUI testing, especially the model-based test generation.
For example, the search-based energy testing tool \textit{COBWEB}~\cite{DBLP:conf/icse/JabbarvandLM19} and the asynchronous programming error detecting tool \textit{APEChecker}~\cite{DBLP:conf/kbse/FanSCMLXP18} both generate executable test cases for bug triggering based on the CTG construction.
In addition, ICC resolution is used to generate storyboard for Android apps~\cite{DBLP:conf/icse/ChenFCSLLX19}.
In the above application scenarios, most works directly apply or extend the existing ICC resolution tools.
Considering both the precision and completeness of ICC resolution have great impacts on the effectiveness of higher-level analysis, we take the practical evaluation of ICC resolution techniques as a topic worthy of concern.


\textbf{ICC Resolution Techniques.} 
The pioneering ICC resolution tool \textit{Epicc} \cite{DBLP:conf/uss/OcteauMJBBKT13} first concentrated on this task and reduced the discovery of ICC to an instance of the IDE problem.
It adopted string analysis and performed IDE analysis to compute the values of Intent fields, which are the basis of ICC resolution.
Then \textit{IC3} optimized the approach by defining a declarative language to specify multi-valued composite constant propagation problems and implemented a solver for them.
By now, \textit{IC3} is the most widely used ICC resolution tool.
Recently, several works focused on the improvement of it to recognize more links, e.g., tool \textit{StoryDroid} enhanced \textit{IC3} by adding fragment and inner class handling, \textit{IC3-DIALDroid}~\cite{DBLP:conf/ccs/BosuLYW17} implemented incremental callback analysis and replaced the original one.
Tool \textit{RAICC} reconstructed atypical ICCs to normal ones based on the results of \textit{IC3} to lessen the number of FNs.
Also, \textit{Primo} improved the ICC matching ability by introducing a probability model as a post-processor, which associated probability values to each potential link to remove the FP links.
These works aim to enhance the ability of the existing ICC resolution tools in various aspects.
Compared to them, our work makes the improvement from another side, i.e., we construct a practical, representative, and reliable oracle for tool evaluation and investigated the characteristics which have high impacts on different ICC resolution techniques.

% EdgeMiner~\cite{DBLP:conf/ndss/CaoFBEKVC15} is a call graph edge miner tool, which automatically detecting implicit control flow transitions through the Android framework.
% Although it does not perform ICC resolution, the call edge analysis evaluation could be referred.
% In this work, it evaluates the false positive by manually analyze more than 200 edges and verify ten implicit resgister-callback pairs by instrumentation.
% It also instruments the dalvik Virtual machine to evaluate the false negative by dynamic log analysis.


% The resolution of ICC links (identification of the source and target components, type of the components, etc.) is a well- studied topic in the literature. 

